Practical Attacks Against Graph-based Clustering

Graph modeling allows numerous security problems to be tackled in a general way, however, little work has been done to understand their ability to withstand adversarial attacks. We design and evaluate two novel graph attacks against a state-of-the-art network-level, graph-based detection system. Our work highlights areas in adversarial machine learning that have not yet been addressed, specifically: graph-based clustering techniques, and a global feature space where realistic attackers without perfect knowledge must be accounted for (by the defenders) in order to be practical. Even though less informed attackers can evade graph clustering with low cost, we show that some practical defenses are possible.

==> generalize.tex <==
\section{Working With Different Graph Mining Techniques}

In the previous section, we have shown that the noise injection and diffusion
attacks are effective against the spectral clustering component of the DGA
detection system. The attacks change graph properties by either generating or
removing edges in the NXDomain and host bipartite graph.  This can be
problematic for not only spectral clustering, but also other clustering methods
using graph representations. In this section, we will show that the two
proposed attacks can be generalized to other unsupervised learning techniques
that use graph methods. Specifically, community
discovery~\cite{blondel2008fast} and the node2vec~\cite{grover2016node2vec}
graph embedding technique.

%{\red we need to be consistent about knowledge level here.}

\subsection{Community Discovery}

\paragraph{Noise Injection}

Instead of spectral clustering, we use a community discovery
algorithm~\cite{blondel2008fast} to act as the unsupervised part of Pleiades.
We chose the best partition as communities, then used the classifier to predict
whether each community is likely a DGA class. 
Next we try to attack these good communities using
our ``noise injection attack'' under the minimal knowledge assumption.

\begin{figure}[t]
	\centering
        \subfloat[Prediction Confidence]
        {\includegraphics[scale=0.35]{figures/prediction_confidence_comm_n2v}
        \label{fig:prediction_confidence_comm_n2v}}
        ~
        \subfloat[Anomaly cost.]
        {\includegraphics[scale=0.35]{figures/uniqnxnum_percentile_n2vcomm}
        \label{fig:uniqnxnum_percentile_comm_n2v}}
        \caption{ Figure~\ref{fig:prediction_confidence_comm_n2v}: Prediction confidence
        before attack, and after noise injection using benign DGA
        for community discovery and node2vec.
        Figure~\ref{fig:uniqnxnum_percentile_comm_n2v}: Percentile of
        unique NXDomain numbers increase.}
        \label{fig:noiseinjection_n2vcomm}
\end{figure}


% no noise ratio

We inject one benign DGA domain every time an adversary's DGA domain is
queried. Then we measure the classification confidence of adversarial clusters.
Figure~\ref{fig:prediction_confidence_comm_n2v} shows the classification confidence for the Pykspa
cluster before the attack, and the median confidence for the resulting
adversarial clusters after the attack. Before the attack, the confidence ranged
from {\red AA}\% to {\red BB}\%. After the attack, \yizheng{..}.
This demonstrates that noise injection attack is effective against community
discovery algorithm.

% doing diffusion attack for community discovery does not worth the cost.

\paragraph{Diffusion} % (fold)
\label{par:Diffusion}

\yacin{Please help with this argument.}
Islands are different communities. So the cost of diffusion attack is highest
because it needs to generate singletons.

% paragraph Diffusion (end)

\subsection{node2vec}
\label{section:node2vec}


\begin{figure}
    \centering
    \scalebox{0.3}{\includegraphics{figures/context_size_l80}}
    \caption{
    Use cluster validity metrics to choose context size. We use context
    size 6.
    }
   \label{fig:valitiy_contextsize}
\end{figure}


\begin{figure}
    \centering
    \scalebox{0.3}{\includegraphics{figures/walk_length_wnum}}
    \caption{
    Use cluster validity metrics to choose walk length. We use walk
    length 20.
    }
   \label{fig:valitiy_walklength}
\end{figure}

\begin{figure}
    \centering
    \scalebox{0.3}{\includegraphics{figures/walk_number_k6}}
    \caption{
    Use cluster validity metrics to choose number of walks per node. We use
    15 walks per node.
    }
   \label{fig:valitiy_walknum}
\end{figure}

\yizheng{fill out details.}
We first chose context size according to Figure~\ref{fig:valitiy_contextsize}.
Then we chose length of walk according to Figure~\ref{fig:valitiy_walklength}.
Then we chose number of walks per node according to Figure~\ref{fig:valitiy_walknum}.
These two don't have much different: dimenions 60 and epoch 1.
We use uniformly random probability to choose each next node in the random walk.

\paragraph{Noise Injection} % (fold)
\label{par:Noise Injection}

Figure~\ref{fig:prediction_confidence_comm_n2v}. \yizheng{fill out details.}

% paragraph Noise Injection (end)

\paragraph{Diffusion Attack}

It is a limitation of the spectral decomposition of a graph in a continuous
feature space that information about small components of the graph is lost.  A
newer graph embedding technique, node2vec, improves upon the spectral
representation method. We show that our death star attack is still effective
against the latest node2vec technique, although the cost of launching the
attack is higher in node2vec than in the spectral decomposition case.

\begin{figure}[t]
	\centering
        \subfloat[Weighted percentage of noisy domains in adversarial DGA clusters.]
        {\includegraphics[scale=0.2]{figures/n2v_diffusion_wfrac_r15}
        \label{fig:n2v_wfrac}}
        ~
        \subfloat[Maximum confidence of prediction after diffusion attacks.]
        {\includegraphics[scale=0.2]{figures/n2v_diffusion_r15}
        \label{fig:n2v_maxprob}}
        \caption{Diffusion attack can succeed in node2vec.}
        \label{fig:n2v_diffusion}
\end{figure}

\begin{figure}[t]
    \centering
    \scalebox{0.48}{\includegraphics{figures/n2v_maxprob_multiplot_contextsize_success}}
    \caption{Success area of diffusion attack with different context size.
    Instead of context size 6,
    this indicates we should choose 2 or 4.}
    \label{fig:n2v_maxprob_multiplot_contextsize}
\end{figure}


\begin{figure}[t]
    \centering
    \scalebox{0.48}{\includegraphics{figures/n2v_maxprob_multiplot_walklength_success}}
    \caption{Success area of diffusion attack with different length of walks.
    Instead of walk length 20,
    this indicates we should choose length 12. }
    \label{fig:n2v_maxprob_multiplot_walklength}
\end{figure}

% introduce node 2 vec

node2vec uses a combination of a random walk with the
Word2Vec~\cite{mikolov2013efficient} latent embeddings to represent
neighborhoods of each node on the graph in continuous feature space. 
We used hyperparamters chosen by aforementioned cluster validity method. 
By clustering using vectors generated by node2vec,
there is not a large death star, since the walk length forces a smaller
neighborhood, but rather there are a few mixture clusters that include a large
variety of domains.  Small components of the graph are in these mixture
clusters. The few most popular NXDomains can form their own cluster through
node2vec representation.

We choose the same DGA cluster with 618 domains to
generate adversarial instances. We wish to break down the cluster into small
components and see if it is possible to make the domains join the mixture
clusters.  Figure~\ref{fig:n2v_diffusion} shows that diffusion
attack is still possible. Figure~\ref{fig:n2v_wfrac} shows the weighted percentage of noise in
related clusters with adversarial DGA. Figure~\ref{fig:n2v_maxprob} shows
the maximum prediction confidence for any of the adversarial clusters
after diffusion attack. The white spaces mean none of the adversarial clusters
under that configuration can be predicted.

\yizheng{fill out details.}
Figure~\ref{fig:n2v_maxprob_multiplot_contextsize} and Figure~\ref{fig:n2v_maxprob_multiplot_walklength}
shows success area and cost of attacks change when hyperparamters change.



==> guidedwalk.tex <==
\subsection{Combine Clustering with Classification}

The problem with our spectral clustering is that there is no good
definition of ``similarity'' between domains when we clustering
the entire bipartite graph of hosts and NXDomains they queried.
Node2Vec performs better than spectral clustering because it defines
a neighborhood for each domain. Under walk length 4, it means
the neighborhood is refined in four hops away from itself, equivalent
to two reflections of related hosts and other domains they queried.
This is an improvement over spectral clustering, but not a sufficient
definition of similarity to apply to DGA detection. Thus, Node2Vec is
still vulnerable to noise injection attack and diffusion attack.

Our idea to mitigate these problems is to combine clustering with
classification. We aim to incorporate DGA features in the process
of clustering, in order words, to add domain name characteristics
to the definition of "similarity" in addition to structure of the bipartite
graph. Specifically, we are going to de-randomize Node2Vec. Instead
of doing random walk to find the neighborhood of each domain,
we are going to do a guided walk. Direction of the walk can be determined
by:
\begin{itemize}
\item Edit distance of two domains
\item A prior probability that two domains belong to the same DGA.
\end{itemize}

We are going to build this improved DGA detection system, have a good
detection accuracy and low false positive rate, then evaluate it
again with noise injection attack and diffusion attack.

To generalize the idea, combining clustering with classification should
be considered in other applications as well.


==> overview.tex <==
\section{Overview} % (fold)
\label{sec:Overview}

Prior work in adversarial machine learning in security have focused primarily
on supervised learning and at the system-level, such as classifying PDF malware
or evading image classification systems. The next step is two-fold: to
understand how attackers can evade unsupervised systems where a label---such as
\emph{malicious} or \emph{benign}---is not known ahead of time and identify
differences when features are extracted from a subset of a global Internet,
versus local. Attacker, botmaster, and adversary are used interchangeably in
the remainder of the paper.

\subsection{Unsupervised Learning} % (fold)
\label{sub:Unsupervised Learning}

\emph{Unsupervised learning}, or \emph{clustering}, is the machine learning
task of grouping together similar training samples present in a dataset
\emph{without} labels. Conversely, \emph{supervised learning}, or
\emph{classification}, is grouping training samples with labels into a fixed
set of classes. While classification tasks abound in security, clustering is
commonly used as well.  In particular, many data-driven security detection
systems use a clustering to discover potential threats, commonly referred to as
\emph{knowledge discovery}, and then classification to find malicious
activities. For instance, DGA domain detection~\cite{pleiades,
chen2016financial}, malware family discovery~\cite{rieck2011automatic},
detecting social engineering download attacks~\cite{nelms2016towards},
enterprise security log analysis~\cite{lioperational}, and malware distribution
detection~\cite{invernizzi2014nazca} all rely on an initial phase of
unsupervised learning. Furthermore, existing work often uses clustering to
bootstrap the system in the cases of malware signature
generation~\cite{perdisci2010behavioral}, feature engineering~\cite{notos,
nelms2013execscent, tamersoy2014guilt}, long-term ad fraud C\&C
analysis~\cite{sinkanalysis}, ease of spam monitoring
effort~\cite{hao2009detecting}, and suspicious outlier
detection~\cite{yen2013beehive}. This points to a need to understand the
potential attacks against unsupervised learning and its impact on knowledge
discovery and subsequent classification accuracy. We focus on attacking the
unsupervised phase of a machine learning system that uses clustering to perform
knowledge discovery in order to render the subsequent classification phase
ineffective.

% subsection Unsupervised Learning (end)

\subsection{Learning with Network Features} % (fold)
\label{sub:Learning with Network Features}

Attacking machine learning based on features extracted from the network
presents additional challenges not seen elsewhere because the behavior from
which features are extracted is global. First, manipulating network behavior as
a botmaster can have dire effects on an infection, such as losing network
connectivity to one's botnet or making communication a noticeable outlier,
which make automatically identifying adversarial instances difficult. Second,
while the behavior itself is global, network operators and malware authors
typically only have a subset of this view, which further complicates the
ability to evade a machine learning system. More difficult still, there is no
guarantee that a botmaster's and defender's visibility overlap except on
machines under a botmaster's control. To address this, we consider adversaries
with varying levels of knowledge of the Internet with respect to the defenders
that have built such a system.

% subsection Learning with Network Features (end)

\subsection{Threat Model} % (fold)
\label{sub:Threat Model}

We assume attackers at all knowledge levels have at least one active infection
in one or more networks under analysis by the defender. The attacker is capable
of using any information that could be gathered from their infected hosts to
aid in their adversarial attacks. We also assume that an attacker has black-box
access to the target classifier or an accurate, surrogate classifier that
approximates the accuracy and behavior of the true classifier used by the
defender based on publicly available datasets. Finally, an attacker has full
knowledge of the features, machine learning models, and hyperparameters used in
both the unsupervised and supervised phases of the machine learning system
under attack as these are often published. Due to the global nature of the
network feature space, we consider three classes of adversary that have
minimal, moderate, and perfect knowledge with respect to the defender's view of
the Internet. This view is based on the networks they construct their training
and testing datasets from.

The attacker's goal is to poison the unsupervised phase of a machine learning
system to evade being classified as malicious. This is accomplished with one of
two attacks: \emph{noise injection} or \emph{diffusion}. In the first attack,
noise is injected into communication by the botmaster's infected hosts to lower
the confidence and classification accuracy of their clustered infrastructure.
In the second attack, the botmaster removes enough network communication to
still maintain control of their infrastructure, but to confuse the clustering
to subdivide their attack infrastructure and lower the subsequent classifier's
accuracy. Both attacks are explained in additional detail in
Section~\ref{section:evasion}.

\paragraph{Minimal Knowledge} % (fold)
\label{par:Minimal Knowledge}

The minimal knowledge case represents the least sophisticated adversary. In
this case, the botmaster can only rely on network traffic that can be collected
from their own infected hosts and any publicly available, open source
intelligence (OSINT). For example, the attacker can use OSINT to select
potential network data to inject as noise, coordinate network activity across
infections to appear to be unrelated infections, or masquerade as publicly
known, legitimate network services. An attacker with minimal knowledge is
similar to an average botmaster.

% paragraph Minimal Knowledge (end)

\paragraph{Moderate Knowledge} % (fold)
\label{par:Moderate Knowledge}

% Note from Yacin: we currently don't check this at different levels, but it
% would be a good experiment to add. Keep this in mind.

The moderate knowledge case represents an adversary with additional network
data to construct surrogate models. In addition to OSINT data and network
traffic from their infected hosts, the moderately sophisticated botmaster also
has a full network dataset from a large enterprise or university to approximate
the view of the defender. This allows the adversary to perform their own
clustering and evaluate their attacks more thoroughly. The underlying
assumption of the moderate knowledge attacker is a large network dataset will
enable a stronger likelihood of evading successful detection by the defender.
We will evaluate this using a large university network that supports
approximately 60,000 students, faculty and administrative staff.  We will
randomly sample traffic from this network dataset to approximate the benefit of
the moderate knowledge attacker using smaller networks. An attacker with
moderate knowledge is similar to a sophisticated botmaster with access to a
regional Internet service provider or large network through legitimate or
illegitimate means.

% paragraph Moderate Knowledge (end)

\paragraph{Perfect Knowledge} % (fold)
\label{par:Perfect Knowledge}

Finally, the perfect knowledge case is for an adversary that has obtained the
very network dataset the defenders use to build their models. Given the full
dataset and knowledge of the modeling process, an adversary can completely
reconstruct the clustering and classification results of the defender to
evaluate the effectiveness of their evasion attacks. Ideally, this data would
be well guarded making this level of knowledge only realistic for the most
sophisticated of attackers, e.g., nation-state sponsored threats.

% paragraph Perfect Knowledge (end)

% subsection Threat Model (end)

To evaluate the potential of adversarial attacks on unsupervised learning, we
choose to build proof-of-concept attacks and defenses for an implementation of
Pleiades~\cite{pleiades}, a domain-name generation algorithm (DGA) detection
system. Pleiades makes for a good case study because it is a network-based
detector and relies on clustering. First, by using network data, the features
are global which requires us to understand the knowledge level of attackers.
Second, the knowledge discovery clustering step directly feeds into the
classification step, which provides a convenient measure for adversarial
success when evading the unsupervised component.

% section Overview (end)


==> related.tex <==
\section{Related Work on Adversarial Machine Learning}


\subsection{DGA Detection Systems}

% Main features. How people discussed evasion problems in these papers.
% How do they define a group of domains? Do they need to use clustering?
DGA detection systems that mine network traffic have a similar
structure of first grouping domains together and second
characterizing the groups.
% mining network traffic.
Pleiades~\cite{pleiades} uses a combination of clustering and classification algorithms to
detect DGA families. It utilizes two clustering algorithms, one using domain name statistical features
and the other using spectral clustering of bipartite graphs.
The intersections of two clustering results are used for classification.
The classification phase has two statistical models to predict new DGA families
using domain name string statistical features.
One is a multi-class Alternating Decision Trees model to classify groups
of DGA domains. The other is distinct Hidden Markov Models for each DGA to
predict individual DGA domain.
We built a simplified version of Pleiades~\cite{pleiades}. Our system has only
one spectral clustering component and one classification model to predict
each cluster. We excluded multiple filtering steps from the original Pleiades
to eliminate trivial adversarial evasion instances that can make DGA domains
being filtered out by the system, with the goal of
focusing on adversarial analysis of the clustering and classification algorithms.
Phoenix~\cite{schiavoni2014phoenix} uses a joint clustering and fingerprinting
approach to characterize DGA families from blacklisted and low-reputation domains.
The clustering process uses resolved IP address features to form a bipartite graphs for
candidate domains, and does spectral clustering of the graph. The fingerprinting process
uses domain name string statistical features and IP address features as signatures
for clusters. Dictionary DGAs can evade Phoenix
because it filtered out all domains with pronounceable English words.
Yadav et al.~\cite{yadav2010detecting} proposed methodology to detect
algorithmically generated domains by first grouping domains together and then
computing features of domains in the group to classify DGAs.
They group domains that point to the same top level domains, same IP address,
or form a connected component in the domain-IP resolution graph.
All of the three systems used statistical features in domain strings
when they classifies or characterizes groups of domains. For instance,
length, one-gram set, top level domains, number percentage, and n-gram features.

% Botnet analysis
% reverse engineer malware.
Previous work that detect DGA domains are have also used botnet analysis
and malware analysis methods.
Chen et al.~\cite{sinkanalysis} used spectral clustering with label propagation
techniques to analyze the ad fraud activity of TDSS/TDL4 which used a server-side
DGA. Stone-Gross et al.~\cite{stone2009your} reverse engineered
Torpig botnet DGA algorithm.
Plohmann et al.~\cite{plohmann16comprehensive} studied DGA algorithms
by reverse engineering 43 malware families.
Rossow et al.~\cite{rossow2013sok} revealed that Zeus used a DGA as backup
Command \& Control (C\&C) mechanism by reverse engineering.
Neugschwandtner et al.~\cite{neugschwandtner2011detecting} implemented
a multi-path exploration technique for dynamic malware anlaysis, which
can trigger failover DGA C\&C for bots.



\subsection{Adversarial Machine Learning}

% adversarial classification
{\red Reduce.}
Most existing work focused on analyzing the security properties of classifiers.
%such as spam filters, phishing page detection, antivirus software, local
%network intrusion detection and anomaly detector. Many of these systems are
%vulnerable to adversarial attacks.
Huang et al.~\cite{huang2011adversarial} categorize attack influence as
\emph{causative} or \emph{exploratory}.
%The work also proposes taxonomies for
%security violation achieved by the attacks, and the specificity of the attacks.
\emph{Causative} attacks aim to alter the training dataset in order to influence
the model. For instance, researchers have studied
attacks and defenses to pollute automatic signature
generation~\cite{newsome2006paragraph, venkataraman2008limits,
chung2006allergy, chung2007advanced, rubinstein2009antidote, perdisci2006misleading},
attacks against spam detection~\cite{nelson2008exploiting, nelson2009misleading,
dalvi2004adversarial}, poisoning anomaly detector to let
DoS attack go undetected~\cite{rubinstein2009antidote}, etc.
On the contrary, \emph{exploratory} attacks do not have the ability to
contaminate the training dataset. Instead, exploratory attacks try to unveil
information about the training data by probing the detector. In order to make
bad activities look like good activities, generally attackers use methodology of
enhancing ``benign features'' and reducing ``malicious features''.
For example, polymorphic blending attack~\cite{fogla2006evading}
uses polymorphic instances that are
statistically indistinguishable from benign instances to evade intrusion
detection systems.
% image
Feature deletion attacks~\cite{globerson2006nightmare} set
features with big weights to zero values to influence the classifier. Mimicry
attacks~\cite{wagner2002mimicry, tan2002undermining} try to evade intrusion
detection systems by mimicking operations of benign applications. 
Spam good word attack~\cite{lowd2005good, wittel2004attacking} inject good words
to bypass spam filtering. Attack against
PDFRATE~\cite{smutz2012malicious, rndic2014practical, xu2016automatically} add ``benign features".
Rndic et al.~\cite{rndic2014practical} reverse engineered the client-side classifier of
Chromium. They used some ``benign'' features of phishing page background
color to surpass the detector.

Using taxonomy from~\cite{huang2011adversarial}, we consider \emph{exploratory}
attack that attempts to violate the \emph{integrity} of
the system with the goal of making DGA domains appear
normal. The goal of the attack is \emph{targeted}.

% privacy and surrogate model.
If some data samples and their class labels can be obtained (e.g., using
an API), the \emph{privacy} of the ML model can be violated.
Tram{\`e}r et al.~\cite{tramer2016stealing} reliably
extracted popular ML models including linear classifiers, neural networks and decision trees
based on only class labels. Papernot et al.~\cite{papernot2016transferability} studied
model transferability and concluded that adversary can use a different
model as surrogate model given enough data labels.

% knowledge level and cost.
{\red TODO: Knowledge limits.}
Some previous work have discussed attacker's knowledge limits.
Rndic et al.~\cite{rndic2014practical}
mentioned Venn Diagram of training dataset, features and classifier.
Discussion about black-box and white-box...
Exploratory attacks assume black-box, and no access to the training data.
Knowledge about the features is strong enough.
% does pollution attack assume access to the training dataset?

{\red TODO: Cost.} Previous work dealt with direct feature manipulation.
Lowd et al.~\cite{lowd2005adversarial} proposed a linear cost function for crafting evasive adversarial
samples. An adversary wants to minimize the cost of changing
feature values from a malicious instance in order for it to be classified as benign.
%The paper
%uses spam filter with uniform cost per feature as example, and conducted experiments
%to show that greedily changing a feature with the largest weight-to-cost ratio can successfully
%vade a linear classifier. This paper also does not assume perfect knowledge, but rather gives
%a polynomial-time algorithm (oracle queries) for the adversary
%to approximate the weights of linear classifiers.
Laskov et al. and Nelson et al.~\cite{laskov2009framework, nelson2006bounding} used
multi-dimentional hypersphere to illustrate \emph{bounds} of successful
attack.


% adversarial clustering
{\red TODO: cite two early ones about adversarial clustering.}
Biggio et al.~\cite{biggio2013data} studied taxnomoy of adversarial clustering.
{\red talk about their "bridge" method.}
%maximal difference of two sets of
%clusters, as some optimization problem.
They applied the attack to malware clustering~\cite{biggio2014poisoning},
assuming perfect knowledge of the attacker.
In comparison, we discuss different knowledge levels, and also add a classification
component of the system, to show how adversarial clustering affects the whole system.




==> supervised.tex <==


